Modelling sand ripples in mine countermeasure simulations by means of stochastic optimal control

Modelling and simulating mine countermeasures (MCM) search missions performed by autonomous vehicles equipped with a sensor capable of detecting mines at sea is a challenging endeavour. In this work, we present a novel way to model and account for sand ripples present on the bottom of the ocean while calculating trajectories for the autonomous vehicles by means of a stochastic optimal control framework. It is known from the scientific literature that these ripples impact the sea mine detection capabilities of the autonomous vehicles.

==> coverage_80.tex <==

\begin{tikzpicture}

    \node at (3.5,6.5) {\large Coverage: 80\%};

\end{tikzpicture}

